Optimality of Sub-network Laplace Approximations: New Results and Methods

Although the Laplace approximation offers a simple route to uncertainty quantification in deep neural networks, its reliance on inverting large Hessian matrices has motivated a range of computationally feasible low-dimensional or sparse approximations. A prominent class of such methods - sub-network Laplace approximations, constructs surrogates by restricting attention to a small subset of parameters. Existing approaches in this family typically rely on diagonal, layer-wise, or other architectural heuristics for subset selection, which ignore cross-parameter interactions and lack formal optimality guarantees. In this paper, we provide a rigorous theoretical analysis of the sub-network Laplace paradigm. We prove that all sub-network Laplace methods systematically underestimate the predictive variance of the full Laplace posterior, and that this bias decreases monotonically as the retained sub-matrix expands. Leveraging this insight, we propose two principled, analytically grounded sub-network Hessian approximations: \textit{Gradient-Laplace} selects parameters with the largest average squared gradients of the model output with respect to the parameters over a reference dataset; while \textit{Greedy-Laplace} iteratively refines this selection by accounting for off-diagonal interactions in the precision matrix. We establish theoretical guarantees characterizing their optimality properties and show that Gradient-Laplace provably outperforms existing heuristic approaches. Extensive numerical studies across diverse settings indicate that these methods perform strongly relative to existing benchmarks.

==> wass_real_main.tex <==
% =====================================================================
% Drop-in replacement for §5.1 ("Experiment 1: Accuracy of Sub-network
% Selection", \label{subsec:Simulation_wass}) in `Posterior Approx Update.tex`.
%
% Replaces the synthetic well-/mis-specified setup with two real-world
% benchmarks: YEAR Prediction MSD (regression) and a binary reduction of
% CIFAR-10 (classification). The accompanying figures are 2-panel layouts
% covering both the §5.1 W_2 metric (left) and the §5.2 coverage metric
% (right), shared between Sections~\ref{subsec:Simulation_wass} and
% \ref{subsec:simulation_cover}.
%
% Use:  \input{wass_real_main}   (no .tex extension needed)
%
% Cross-references used (must already exist in the host file):
%   \eqref{posterior:predictive:variance} — regression predictive (Eq. 3)
%   \eqref{Gauss:Newton:precision}        — regression precision (Eq. 2)
%   \eqref{Gen_Gauss:Newton:precision}    — generalized GGN (Eq. 4 / binary)
%   \ref{thm1}                            — Theorem 1
%   \ref{thm2}                            — Theorem 2 (Subnet Diagonal worst)
%   \ref{subsec:simulation_cover}         — §5.2 coverage subsection
%   \ref{app:wass_real}                   — appendix label (in wass_real_appendix.tex)
%   \ref{app:benchmark_algo}              — benchmark algorithm appendix
%
% Figure paths used in main (copy these into the host paper's image dir):
%   Plots/year_paper_figure_ci.png         — YEAR W_2 + CI coverage (2-panel)
%   Plots/paper_figure1_binary_resnet110.png — CIFAR-binary R110 (headline)
%
% Additional figures referenced from the appendix (wass_real_appendix.tex):
%   Plots/paper_figure1_binary_resnet20.png  — Appendix scaling block (top)
%   Plots/paper_figure1_binary_resnet32.png  — Appendix scaling block (middle)
%   Plots/paper_figure1_binary_resnet56.png  — Appendix scaling block (bottom)
%   Plots/wasserstein_uci.png                — Appendix Setup D figure
% =====================================================================

\subsection{Experiment 1: Accuracy of Sub-network Selection}
\label{subsec:Simulation_wass}

\noindent
\textbf{Experimental Setup}. To quantify the quality of subnetwork-based approximations, \citet{daxberger2021bayesian} suggest using the Wasserstein distance between the full linearized Laplace posterior for $\bm{\theta}$ with covariance $\Omega^{-1}$ and the corresponding \textit{sub-network LA} surrogate, given by a singular multivariate Gaussian with covariance $([\Omega_{S,S}]^{0})^{-}$, the Moore--Penrose pseudo-inverse of $[\Omega_{S,S}]^{0}$. To measure the predictive consequences of this matrix-level mismatch we report, at each test input $\mathbf{x}^{*}$, the Wasserstein-2 distance between the predictive distribution at $\mathbf{x}^{*}$ implied by~\eqref{posterior:predictive:variance} and its surrogate counterpart. Since both predictive distributions are Gaussian with the same mean, this collapses to $|\sigma_{\mathrm{Full}}(\mathbf{x}^{*}) - \sigma_{\mathrm{method}}(\mathbf{x}^{*})|$, the absolute predictive-standard-deviation gap. We compare the proposed \emph{Gradient-Laplace} and \emph{Greedy-Laplace} subnetworks against the existing \textit{sub-network LA} benchmarks \emph{Subnet Diagonal}~\citep[Section 5]{daxberger2021bayesian} and \emph{NeuralLinear}~\citep{snoek2015scalable,riquelme2018deep}, the natural \emph{Last $k$} extension of NeuralLinear (Appendix~\ref{app:benchmark_algo}), and the non--\textit{sub-network LA} baseline \emph{PrecisionDiag}~\citep{riquelme2018deep,zhang2020neural}. On the regression coverage panel (Setup A) we additionally overlay a \emph{Deep Ensemble} baseline~\citep{lakshminarayanan2017simple}, drawn as a $k$-independent horizontal reference. Definitions of all benchmark algorithms are provided in Appendix~\ref{app:benchmark_algo}.

To exercise the proposed methods at a scale and in modeling regimes that are representative of practical Bayesian deep learning, we evaluate on two real-world benchmarks: a high-dimensional tabular regression task and a deep image-classification task. Their selection is deliberate: the first targets the regression formulation in~\eqref{posterior:predictive:variance}--\eqref{Gauss:Newton:precision}, while the second targets the binary-classification generalization with the scalar-Hessian Gauss--Newton precision in~\eqref{Gen_Gauss:Newton:precision}. Together they exercise both forms of the predictive variance under which our theoretical guarantees were derived, on backbones spanning $p \approx 10^{5}$ (YEAR; Setup A) and $p \approx 2.7 \times 10^{5}$ to $1.7 \times 10^{6}$ (Binary CIFAR-10 with ResNet-20 through ResNet-110; Setup B).

\noindent
\textbf{Setup A: YEAR Prediction MSD (regression).} The \emph{YearPredictionMSD} dataset~\citep{bertinmahieux2011yearpredictionmsd} from the UCI repository is a standard large-scale tabular regression benchmark in which the task is to predict a song's release year from $90$ timbre features. We use the canonical train/test split with target standardization fit on the training partition only. The working model is a 3-hidden-layer width-$200$ ReLU MLP with a scalar linear head ($p = 98{,}801$ parameters), trained with the mean squared error loss for $100$ epochs.

\noindent
\textbf{Setup B: Binary CIFAR-10 (classification).} The CIFAR-10 dataset~\citep{krizhevsky2009learning} is a standard $32 \times 32$ colour-image classification benchmark with ten classes. We construct a balanced binary task by collapsing the ten labels into two groups of five via $y_{\mathrm{binary}} = \mathbf{1}\{y \geq 5\}$. The working model is a CIFAR-style ResNet~\citep{he2016deep} in which the standard $\mathrm{Linear}(64, 10)$ head is replaced by a single-output $\mathrm{Linear}(64, 1)$ logit; we evaluate the full four-member family ResNet-20 / 32 / 56 / 110 (head-swapped parameter counts $p = 271{,}889 / 466{,}906 / 855{,}930 / 1{,}730{,}129$) and report the largest member, ResNet-110, in the headline figure. Training uses the binary cross-entropy loss for $100$ epochs under the standard CIFAR-10 SGD recipe. Under this reduction, the Gauss--Newton precision matrix specializes to~\eqref{Gen_Gauss:Newton:precision} with a scalar per-sample Hessian factor $p_{n}(1 - p_{n}) = \sigma(f_{\bm{\theta}}(\mathbf{x}_{n}))(1 - \sigma(f_{\bm{\theta}}(\mathbf{x}_{n})))$, so all subnetwork-LA computations reuse the regression machinery on a sqrt-Hessian-weighted training Jacobian $J_{w}[n] = \sqrt{p_{n}(1 - p_{n})}\, J(\mathbf{x}_{n})$.

For both setups, the per-sample Wasserstein metric is averaged over a fixed test subsample, and we report the mean and standard error over ten independent random seeds. The same trained MAP estimate is shared across all subnetwork-LA methods within a given seed; only the index set $S$ differs between methods. Full architecture and hyperparameter details, the protocol for the oracle target $f_{\bm{\theta}_{0}}$ used in the coverage panels, and the precision matrix specialization in Setup B are in Appendix~\ref{app:wass_real}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{year_paper_figure_ci.png}
    \caption{Setup A (\textbf{YEAR Prediction MSD}, regression, $p = 98{,}801$). \textbf{Left:} per-test-point average Wasserstein distance between the full Laplace predictive and its sub-network surrogate, as a function of subset size $k$ (log-log axes; lower is better). \textbf{Right:} empirical coverage of the $95\%$ posterior predictive credible interval, as a function of $k$ (log-x axis; the dashed horizontal line marks the nominal $0.95$ level). Lines are means over ten independent random seeds and shaded bands show one standard error. The dash-dotted horizontal line marks the \emph{Deep Ensemble}~\citep{lakshminarayanan2017simple} coverage at $M = 10$ ensemble members, trained with the same architecture, recipe, and seed-set as the LA suite. The right panel is reproduced and discussed in Section~\ref{subsec:simulation_cover}.}
    \label{fig:wass_year}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{paper_figure1_binary_resnet110.png}
    \caption{Setup B (\textbf{Binary CIFAR-10}, ResNet-110, $p = 1{,}730{,}129$). \textbf{Left:} per-test-point average Wasserstein distance between the full Laplace predictive and its sub-network surrogate, as a function of subset size $k$ (log-log axes; lower is better). \textbf{Right:} empirical coverage of the $95\%$ posterior predictive credible interval, as a function of $k$ (log-x axis; the dashed horizontal line marks the nominal $0.95$ level). Lines are means over ten independent random seeds and shaded bands show one standard error. The smaller members of the ResNet family (ResNet-20 / 32 / 56) are reported in Appendix~\ref{app:wass_real:scaling}. The right panel is reproduced and discussed in Section~\ref{subsec:simulation_cover}.}
    \label{fig:wass_cifar_binary}
\end{figure}

\noindent
\textbf{Results and Discussion}. Figures~\ref{fig:wass_year} and~\ref{fig:wass_cifar_binary} report the Wasserstein metric (left panels) on the YEAR regression setup and on the headline Binary CIFAR-10 ResNet-110 setup. The corresponding curves at the smaller backbones ResNet-20 / 32 / 56 are reported in Appendix~\ref{app:wass_real:scaling}. Across both setups and across the full subset-size grid, the proposed \emph{Gradient-Laplace} and \emph{Greedy-Laplace} methods provide a substantially closer approximation to the full Laplace posterior predictive than the existing subnetwork benchmarks \emph{Subnet Diagonal} and \emph{Last $k$}, which remain near their large-$k$ asymptote even as $k$ grows. \emph{NeuralLinear} (the dedicated last-layer subset, $k = 201$ for YEAR, $k = 65$ for the binary CIFAR-10 head) sits at a single fixed subset size and is matched or surpassed by the proposed methods at comparable $k$. This empirical ordering is consistent with the theoretical guarantee in Theorem~\ref{thm1} that selecting parameters by their average squared training Jacobian is asymptotically optimal in our idealized predictive-variance metric, and with the negative result in Theorem~\ref{thm2} which excludes the smallest-diagonal selection rule from this optimum.

On the headline Binary CIFAR-10 ResNet-110 panel (Figure~\ref{fig:wass_cifar_binary}, $p \approx 1.7 \times 10^{6}$) a clear secondary trend emerges: \emph{Greedy-Laplace} sits below \emph{Gradient-Laplace} at every $k$ in the grid, with the gap most pronounced at moderate-to-large $k$. The four-backbone scaling sweep in Appendix~\ref{app:wass_real:scaling} shows that this advantage grows mildly with $p$: at ResNet-20 the two proposed methods are essentially co-best (curves overlap within their seed-level uncertainty bands), at ResNet-32 / 56 a small consistent gap opens up, and at the headline ResNet-110 it is most visible. This is the regime in which the off-diagonal corrections incorporated by the Schur-complement step of Algorithm~\ref{alg:neuralnet1} are expected to matter most: as $p$ grows past $\approx 10^{6}$, the cross-parameter correlations in $\Omega$ that \emph{Gradient-Laplace} ignores become a more visible fraction of the predictive-variance signal. Throughout this scaling sweep, \emph{Subnet Diagonal} and \emph{Last $k$} remain essentially flat at their MAP-only $W_{2}$.

The right panels of Figures~\ref{fig:wass_year} and~\ref{fig:wass_cifar_binary} display the empirical coverage of the $95\%$ posterior predictive credible interval and are discussed in Section~\ref{subsec:simulation_cover}. The Deep Ensemble overlay on Figure~\ref{fig:wass_year}'s right panel is at $0.99$ coverage, slightly above nominal, and is matched (within seed noise) by \emph{Gradient-Laplace} and \emph{Greedy-Laplace} once $k \gtrsim 10^{4}$. \emph{Subnet Diagonal} systematically under-covers across the full range of $k$ on both setups.

Overall, the real-data experiments on YEAR and Binary CIFAR-10 reproduce the qualitative findings of our synthetic-data analysis at a substantially larger scale, and the four-backbone scaling sweep deferred to Appendix~\ref{app:wass_real:scaling} demonstrates that the proposed subnetwork strategies remain effective --- and the \emph{Greedy-Laplace} refinement increasingly valuable --- at modern depth ($p$ from $\approx 10^{5}$ to $\approx 10^{6}$). The regime $p \gtrsim 10^{6}$ is exactly the one in which the proper multi-class softmax-Hessian formulation of~\eqref{Gen_Gauss:Newton:precision} becomes infeasible at $N = 2{,}000$ on a single H100; the binary reduction makes it tractable to push the comparison to a backbone size that would otherwise be out of reach.

